Invariance in Policy Optimisation and Partial Identifiability in Reward Learning

It is often very challenging to manually design reward functions for complex, real-world tasks. To solve this, one can instead use reward learning to infer a reward function from data. However, there are often multiple reward functions that fit the data equally well, even in the infinite-data limit. This means that the reward function is only partially identifiable. In this work, we formally characterise the partial identifiability of the reward function given several popular reward learning data sources, including expert demonstrations and trajectory comparisons. We also analyse the impact of this partial identifiability for several downstream tasks, such as policy optimisation. We unify our results in a framework for comparing data sources and downstream tasks by their invariances, with implications for the design and selection of data sources for reward learning.

==> figure.tex <==
\begin{figure}[h!]
\begin{center}
\begin{subfigure}{0.5\textwidth}
\begin{tikzpicture}
    % regions
    \node[ellipse,rotate=-10,inner sep=15,minimum width=110,fill=black!5,text=black!70]
        at (6.0,1.3) {IRL};
    \node[ellipse,rotate=-10,inner sep=15,minimum width=110,fill=black!5,text=black!70]
        at (2.0,1.1) {pref. cmp.};
    % axis
    \node[label={[below right,text width=2cm]increasing ambiguity (tolerance)}]
          (label) at ( 0.00, 3.53) {};
    \draw[->] (0.00, 3.80) -- (0.00, 0.40);
    % nodes
    \node (0) at ( 1.00, 3.80) {$\reward$}; % 
    \node (1) at ( 5.00, 3.00) {$Q$};
    % \node (2) at ( 1.00, 3.40) {$\preceq^{\policy}$}; % policy evaluation order node
    \node (3) at ( 5.00, 2.00) {$\MaximumEntropyPolicy$};
    \node (4) at ( 7.00, 1.60) {$\OptimalPolicy$};
    \node (5) at ( 5.00, 1.00) {$\Delta_\beta$};
    \node (6) at ( 7.00, 0.60) {$\Delta_\star$};
    \node (7) at ( 3.00, 3.40) {$\Return_\zeta$};
    \node (8) at ( 3.00, 2.40) {$\Return_\xi$};
    \node (9) at ( 1.00, 1.80) {$\cmpSoftFrag$};
    \node (A) at ( 3.00, 1.40) {$\cmpSoftTraj$};
    \node (B) at ( 1.00, 0.80) {$\cmpStarFrag$};
    \node (C) at ( 3.00, 0.40) {$\cmpStarTraj$};
    % edges
    % \draw[->] (0) -- (2); % policy evaluation arc
    % \draw[->] (2) -- (4); % policy evaluation arc
    % \draw[->] (0) -- (1); % implicit through (0) -- (7) -- (1)!
    \draw[->] (0) -- (7);
    \draw[->] (1) -- (3);
    \draw[->] (3) -- (4);
    \draw[->] (3) -- (5);
    \draw[->] (4) -- (6);
    \draw[->] (5) -- (6);
    \draw[->] (7) -- (1);
    \draw[->] (7) -- (8);
    \draw[<->](7) -- (9);
    \draw[->] (8) -- (A);
    \draw[->] (9) -- (A);
    \draw[->] (9) -- (B);
    \draw[->] (A) -- (C);
    \draw[->] (A) -- (5);
    \draw[->] (B) -- (C);
\end{tikzpicture}
\caption{}
\label{fig:main:reward-functions}
\end{subfigure}
\hspace{0.13\textwidth}%
\begin{subfigure}{0.30\textwidth}
\begin{tikzpicture}
    % corner
    % \node at ( 4.00, 0.00) {};
    % nodes
    \node (0) at ( 2.10, 3.80) {$\mathrm{id}$};
    \node[text width=2cm,align=center]
          (1) at ( 2.10, 2.80) {mask of $\SetComplement{\mathrm{supp}(\TransitionDistribution)}$};
    \node (2) at ( 2.10, 1.60) {$S'$-R.};
    \node (3) at ( 0.60, 2.80) {$k$-$\Phi$};
    \node (4) at ( 0.60, 1.60) {$\Phi$};
    \node (5) at ( 3.70, 2.80) {PLS};
    \node (6) at ( 3.70, 1.60) {ZPMT};
    \node (7) at ( 2.10, 0.60) {OPT};
    % edges
    \draw[->] (0) -- (1);
    \draw[->] (0) -- (3);
    \draw[->] (0) -- (5);
    \draw[->] (1) -- (2);
    \draw[->] (2) -- (7);
    \draw[->] (3) -- (4);
    \draw[->] (4) -- (7);
    \draw[->] (5) -- (6);
    \draw[->] (5) -- (7);
\end{tikzpicture}
\caption{}
\label{fig:main:fundamental}
\end{subfigure}
\end{center}
\caption{
    (a)
    The \emph{infinite-data ambiguity} of reward learning data sources
    and
    the \emph{ambiguity tolerance} of downstream applications of a
    learnt reward function
    are both \emph{invariances} of objects derived from reward functions
    (\cref{sec:prelim,sec:results}).
    %
    These invariances have a \emph{partial order} (\cref{sec:lattice}). Here, $X \rightarrow Y$ means that $Y$ can be derived from $X$, or equivalently, that $Y$ is at least as ambiguous as $X$.
    The objects
    are
    the reward function itself ($\reward$);
    $Q$-functions ($Q$);
    Maximum Entropy ($\beta$) and supportive optimal policies ($\star$) and their induced trajectory distributions ($\MaximumEntropyPolicy$, $\Delta_\beta$ and $\OptimalPolicy$, $\Delta_\star$);
    the return function restricted to partial and full
    trajectories ($\Return_\zeta$, $\Return_\xi$); and
    Boltzmann-distributed ($\beta$) and noiseless ($\star$) comparisons between these trajectories
    ($\cmpSoftFrag$, $\cmpSoftTraj$ and $\cmpStarFrag$, $\cmpStarTraj$).
    % 
    (b)
    Several basic families of reward transformations form the basis
    for our main results (\cref{sec:framework}).
    These transformations exist in a related hierarchy, within (shown here)
    and across tasks (\cref{sec:lattice}).
}
\label{fig:main}
\end{figure}






\newgeometry{left=1.5cm,right=1.5cm,bottom=2.2cm}  % make results page wider to fit table
\section{Directory of results}
\label{apx:directory}

\newcommand{\TI}{\ensuremath{{\equiv}}}
\newcommand{\Ti}{\ensuremath{\TI^{*}}}
\newcommand{\Tx}{\ensuremath{{\times}}}
\newcommand{\TIx}{\Tx/\TI}
\newcommand{\transformationLabel}[1]{%
    \rotatebox{50}{\parbox[c][1.24em]{5em}{%
        \linespread{0.8}\small\selectfont\centering #1}}}
\newcommand{\objectDescription}[1]{\small\raggedright\linespread{0.9} #1}
\newcommand{\prooflink}[1]{%
        \textsuperscript{\hyperlink{#1}{\qedsymbol}}}
\renewcommand{\arraystretch}{1.13} % add a bit of vertical space between rows

\begin{table}[ht!]
    \caption{%
        An overview of the invariance results stated in \cref{sec:results}.
        All proofs are in \cref{apx:proofs}. The lower part lists
        some additional invariance results proved in \cref{apx:proofs}.
        Symbols:
        (\TI) The object is invariant to the transformations;
        (\Ti) The object is invariant to the transformations as a special
        case of the invariances listed in the theorem;
        (\Tx) The object is not generally invariant to the transformations
        (more precisely, it is invariant only to those that can be represented
        as a combination of the listed transformations);
        (\TIx) The extent of the object's invariance to the transformations
        depends on the MDP
        (as in \Cref{thm:labels_of_trajectories}).
        Blank cells indicate unresolved invariances (as in
        \Cref{thm:noiseless-comparisons-trajectories-bound}, see
        also \Cref{remark:noiseless-comparisons-trajectories-bound}).
    }
    \label{table:directory}

    \begin{center}
    \begin{tabular}{cp{9.5em}cc@{\hskip -1.5em}c@{\hskip -1.5em}c@{\hskip -1.5em}c@{\hskip -1.5em}c@{\hskip -1.5em}c@{\hskip -1.5em}c@{\hskip -1.5em}c@{\hskip -1.5em}c@{\hskip -1.5em}c@{\hskip -1.5em}c@{}}
    \toprule
        &&& \multicolumn{11}{c}{Class of transformations}
    \\ \cmidrule(l){4-14}
        \multicolumn{2}{c}{Reward-derived object}
        & \parbox[b]{2.2em}{\centering Thm. \& proof link}
        & \transformationLabel{Identity}
        & \transformationLabel{0-initial $\Phi$ shaping}
        & \transformationLabel{$k$-initial $\Phi$ shaping}
        & \transformationLabel{$\Phi$ shaping}
        & \transformationLabel{S'-redistr.}
        & \transformationLabel{Pos.\ lin.\ scaling}
        & \transformationLabel{ZPMT}
        & \transformationLabel{OPT\\(opt.\ $a$, all\ $s$)}
        & \transformationLabel{OPT\\(opt.\ $a$, opt.\ $s$)}
        & \transformationLabel{Impossible mask}
        & \transformationLabel{Unreachable mask}
    \\ \midrule
        $\reward$
            & \objectDescription{Reward function}
            & --
            & \TI & \Tx & \Tx & \Tx & \Tx & \Tx & \Tx & \Tx & \Tx & \Tx & \Tx
    \\
        $\Qfor{\policy}$
            & \objectDescription{$Q$-function for policy $\policy$}
            & \ref{lemma:Q_function_proximal_redistribution}%
                \prooflink{proof:q}
            & \Ti & \Tx & \Tx & \Tx & \TI & \Tx & \Tx & \Tx & \Tx & \Ti & \Tx
    \\
        $\QStar$
            & \objectDescription{Optimal $Q$-function}
            & \ref{lemma:Q_function_proximal_redistribution}%
                \prooflink{proof:q}
            & \Ti & \Tx & \Tx & \Tx & \TI & \Tx & \Tx & \Tx & \Tx & \Ti & \Tx
    \\
        $\QSoft$
            & \objectDescription{Soft $Q$-function}
            & \ref{thm:soft-q}%
                \prooflink{proof:soft-q}
            & \Ti & \Tx & \Tx & \Tx & \TI & \Tx & \Tx & \Tx & \Tx & \Ti & \Tx
    \\
        $\BoltzmannRationalPolicy$
            & \objectDescription{Boltzmann-rational policy}
            & \ref{thm:boltzmann-rational}%
                \prooflink{proof:boltzmann-rational-policy}
            & \Ti & \Ti & \Ti & \TI & \TI & \Tx & \Tx & \Tx & \Tx & \Ti & \Tx
    \\
        $\MCEPolicy$
            & \objectDescription{MCE policy}
            % & \ref{thm:mce-policy}%
            & \ref{thm:boltzmann-rational}%
                \prooflink{proof:mce-policy}
            & \Ti & \Ti & \Ti & \TI & \TI & \Tx & \Tx & \Tx & \Tx & \Ti & \Tx
    \\
        $\OptimalPolicy$
            & \objectDescription{Maximally supportive optimal policy}
            & \ref{thm:optimal-policies-maximal}%
                \prooflink{proof:supportive-optimal-policies}
            & \Ti & \Ti & \Ti & \Ti & \Ti & \Ti & \Tx & \TI & \Tx & \Ti & \Tx
    \\
        $\TrajDistributionBoltzmann$
            & \objectDescription{Trajectory distribution induced by
                $\BoltzmannRationalPolicy$}
            & \ref{thm:boltzmann-rational-trajectories}%
                \prooflink{proof:boltzmann-rational-trajectories}
            & \Ti & \Ti & \Ti & \TI & \TI & \Tx & \Tx & \Tx & \Tx & \Ti & \TI
    \\
        $\TrajDistributionMCE$
            & \objectDescription{Trajectory distribution induced by
                $\MCEPolicy$}
            % & \ref{thm:mce-trajectories}%
            & \ref{thm:boltzmann-rational-trajectories}%
                \prooflink{proof:mce-trajectories}
            & \Ti & \Ti & \Ti & \TI & \TI & \Tx & \Tx & \Tx & \Tx & \Ti & \TI
    \\
        $\TrajDistributionOptimal$
            & \objectDescription{Trajectory distribution induced by
            $\OptimalPolicy$}
            & \ref{thm:optimal-trajectories}%
                \prooflink{proof:supportive-optimal-trajectories}
            & \Ti & \Ti & \Ti & \Ti & \Ti & \Ti & \Tx & \Ti & \TI & \Ti & \Ti
    \\
        $\Return_\zeta$
            & \objectDescription{Return on possible trajectory
                fragments}
            & \ref{thm:labels_of_fragments}%
              \prooflink{proof:return-fragments}
            & \Ti & \Tx & \Tx & \Tx & \Tx & \Tx & \Tx & \Tx & \Tx & \TI & \Tx
    \\
        $\Return_\xi$
            & \objectDescription{Return on possible, initial
                trajectories}
            & \ref{thm:labels_of_trajectories}%
                \prooflink{proof:return-trajectories}
            & \Ti & \TI & \Tx & \Tx & \Tx & \Tx & \Tx & \Tx & \Tx & \Ti & \TI
    \\
        $\cmpSoftFrag$
            & \objectDescription{Boltzmann comparisons of possible
                fragments}
            & \ref{thm:boltzmann-comparisons-fragments}%
                \prooflink{proof:soft-compare-fragments}
            & \Ti & \Tx & \Tx & \Tx & \Tx & \Tx & \Tx & \Tx & \Tx & \TI & \Tx
    \\
        $\cmpSoftTraj$
            & \objectDescription{Boltzmann comparisons of possible
                initial trajectories}
            & \ref{thm:boltzmann-comparisons-trajectories}%
                \prooflink{proof:soft-compare-trajectories}
            & \Ti & \Ti & \TI & \Tx & \Tx & \Tx & \Tx & \Tx & \Tx & \Ti & \TI
    \\
        $\cmpStarFrag$
            & \objectDescription{Noiseless order of possible fragments}
            & \ref{thm:noiseless-comparisons-trajectory-fragments}%
                \prooflink{proof:hard-compare-fragments}
            & \Ti & \Tx & \Tx & \Tx & \Tx & \TI &\TIx & \Tx & \Tx & \TI & \Tx
    \\
        $\cmpStarTraj$
            & \objectDescription{Noiseless order of possible initial
            trajectories}
            & \ref{thm:noiseless-comparisons-trajectories-bound}%
                \prooflink{proof:hard-compare-trajectories-bound}
            & \Ti & \Ti & \TI &     &     & \TI &     &     &     & \Ti & \TI
    \\
        $\cmpLotteryTraj$
            & \objectDescription{Order of distributions over
                possible initial trajectories}
            & \ref{thm:comparisons-lotteries}%
                \prooflink{proof:compare-lotteries}
            & \Ti & \Ti & \TI & \Tx & \Tx & \TI & \Tx & \Tx & \Tx & \Ti & \TI
    \\
        $\SetOfOptimalPolicies$
            & \objectDescription{Set of optimal policies}
            & \ref{thm:optimal-policies-simple}%
                \prooflink{proof:set-of-optimal-policies}
            & \Ti & \Ti & \Ti & \Ti & \Ti & \Ti & \Tx & \TI & \Tx & \Ti & \Tx
    \\ \midrule
        $\Afor{\policy}$
            & \objectDescription{Advantage function for arbitrary policy
                $\pi$}
            & \ref{lemma:advantage}
            & \Ti & \Ti & \Ti & \TI & \TI & \Tx & \Tx & \Tx & \Tx & \Ti & \Tx
    \\
        $\AStar$
            & \objectDescription{Optimal advantage function}
            & \ref{lemma:advantage}
            & \Ti & \Ti & \Ti & \TI & \TI & \Tx & \Tx & \Tx & \Tx & \Ti & \Tx
    \\
        $\BoltzmannPolicyWrt{\basePolicy}$
            & \objectDescription{Boltzmann policy for arbitrary base policy
                $\basePolicy$}
            & \ref{lemma:boltzmann-general}
            & \Ti & \Ti & \Ti & \TI & \TI & \Tx & \Tx & \Tx & \Tx & \Ti & \Tx
    \\
        $\TrajDistributionBoltzmannWrt{\basePolicy}$
            & \objectDescription{Trajectory distribution induced by
                $\BoltzmannPolicyWrt{\basePolicy}$}
            & \ref{lemma:boltzmann-trajectories-general}
            & \Ti & \Ti & \Ti & \TI & \TI & \Tx & \Tx & \Tx & \Tx & \Ti & \TI
    \\
        \bottomrule
    \end{tabular}
    \end{center}
\end{table}
\restoregeometry
